Multiaccess Channels with State Known to Some Encoders and Independent Messages

We consider a state-dependent multiaccess channel (MAC) with state non-causally known to some encoders. We derive an inner bound for the capacity region in the general discrete memoryless case and specialize to a binary noiseless case. In the case of maximum entropy channel state, we obtain the capacity region for binary noiseless MAC with one informed encoder by deriving a non-trivial outer bound for this case. For a Gaussian state-dependent MAC with one encoder being informed of the channel state, we present an inner bound by applying a slightly generalized dirty paper coding (GDPC) at the informed encoder that allows for partial state cancellation, and a trivial outer bound by providing channel state to the decoder also. The uninformed encoders benefit from the state cancellation in terms of achievable rates, however, appears that GDPC cannot completely eliminate the effect of the channel state on the achievable rate region, in contrast to the case of all encoders being informed. In the case of infinite state variance, we analyze how the uninformed encoder benefits from the informed encoder's actions using the inner bound and also provide a non-trivial outer bound for this case which is better than the trivial outer bound.

==> ltx <==
#!/usr/bin/perl
$a0=shift;

	$comm1=join('',"latex -interaction errorstopmode ",$a0,".tex");
	print "$comm1\n\n";
	system($comm1);
	print "$comm1\n\n";
	$comm4=join('',"latex -interaction errorstopmode ",$a0,".tex");
	print "$comm4\n\n";
	system($comm4);
	print "$comm4\n\n";
	$comm2=join('',"dvips ","-Ppdf -tletter -G0 -q ",$a0,".dvi -o ",$a0,".ps");
	print "$comm2\n\n";
	system($comm2);
	
	$comm3=join('',"gs -q -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -sPAPERSIZE=letter -sOutputFile=",$a0,".pdf ",$a0,".ps");
	print "$comm3\n\n";
	system($comm3);
	

	
#	$comm3=join('',"ps2pdf ",$a0,".ps ",$a0,".pdf");
#	system($comm3);
#	print "$comm3\n\n";


